Constructing and Interpreting Causal Knowledge Graphs from News

Many financial jobs rely on news to learn about causal events in the past and present, to make informed decisions and predictions about the future. With the ever-increasing amount of news available online, there is a need to automate the extraction of causal events from unstructured texts. In this work, we propose a methodology to construct causal knowledge graphs (KGs) from news using two steps: (1) Extraction of Causal Relations, and (2) Argument Clustering and Representation into KG. We aim to build graphs that emphasize on recall, precision and interpretability. For extraction, although many earlier works already construct causal KGs from text, most adopt rudimentary pattern-based methods. We close this gap by using the latest BERT-based extraction models alongside pattern-based ones. As a result, we achieved a high recall, while still maintaining a high precision. For clustering, we utilized a topic modelling approach to cluster our arguments, so as to increase the connectivity of our graph. As a result, instead of 15,686 disconnected subgraphs, we were able to obtain 1 connected graph that enables users to infer more causal relationships from. Our final KG effectively captures and conveys causal relationships, validated through experiments, multiple use cases and user feedback.

==> tabs/patterns.tex <==
\begin{table}[]
\centering
 \resizebox{0.75\columnwidth}{!}{
\begin{tabular}{l}\hline
Causal Linguistic Patterns \\\hline
{[}{[}cause{]}{]}/N -nmod:by   brought/VBN -acl {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nsubj produced/VBD +obj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:by caused/VBN -acl   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:of result/NN -obl   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nsubj results/VBZ +nmod:in   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:from resulting/VBG -acl   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:as listed/VBN   +nsubj:pass cause/NN +nmod:of {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nsubj caused/VBD +obj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:to attributed/VBN   +nsubj:pass {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nsubj lead/VB +nmod:to   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:due occurred/VBD +nsubj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N +acl leading/VBG +nmod:to   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:by caused/VBN +nsubj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N +acl:relcl leads/VBZ +nmod:to   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:with associated/VBN   +conj {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:as reported/VBN   +nsubj:pass cause/NN +nmod:of {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:by cause/VB +obj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:to due/JJ +nsubj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:with associated/VBN   +nmod:of {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N +acl:relcl causes/VBZ +obj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N +acl:relcl resulted/VBD   +nmod:in {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N +conj led/VBD +nmod:to   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nsubj causing/VBG +obj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nsubj led/VBN +nmod:to   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:with associated/VBN   -acl {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nsubj result/VB +nmod:in   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:of result/NN -obl   occurred/VBD +nsubj {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nsubj resulted/VBD +nmod:in   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nsubj triggered/VBD +obj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N +acl:relcl associated/VBN   +nmod:with {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N +acl:relcl produced/VBD +obj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N +acl:relcl brought/VBD +obj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nsubj leads/VBZ +nmod:to   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N +acl:relcl lead/VB +nmod:to   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N +acl causing/VBG +obj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N +acl:relcl led/VBD +nmod:to   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:of result/NN +nsubj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N +acl caused/VBD +obj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N +conj caused/VBD +obj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N +nmod:as cause/NN +nmod:of   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:to attributed/VBD +obj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nsubj brought/VBD +obj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:on blamed/VBD +obj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:due {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N +acl:relcl caused/VBD +obj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N +nsubj causes/NNS +nmod:of   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nsubj causes/VBZ +obj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:to due/JJ -amod   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N +ccomp lead/VB +nmod:to   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nsubj contributed/VBD   +nmod:to {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N +acl resulting/VBG +nmod:in   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nsubj led/VBD +nmod:to   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:of led/VBD +nmod:to   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N +nsubj cause/NN +nmod:of   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:of leading/VBG +nmod:to   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nsubj generate/VB +obj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:with associated/VBN   +obj {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:with associated/VBN   +nsubj {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nsubj lead/VBP +nmod:to   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nsubj cause/NN +nmod:of   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nsubj trigger/VB +obj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N +acl triggered/VBD +obj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:by caused/VBN +nmod:of   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nsubj caused/VBN +obj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:by caused/VBN   +nsubj:pass {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:from resulted/VBD   +nsubj {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -obj followed/VBD +nsubj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:from risk/NN +nmod:of   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nsubj:pass associated/VBN   +nmod:with {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:from occur/VB +nsubj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nsubj cause/VB +obj   {[}{[}effect{]}{]}/N \\
{[}{[}cause{]}{]}/N -nmod:by caused/VBN +obj   {[}{[}effect{]}{]}/N\\\hline
\end{tabular}}
\caption{All linguistic patterns used in our study.
}\label{tab:patterns}
\end{table}

==> tabs/top_patterns.tex <==
\begin{table}[]
\resizebox{1\columnwidth}{!}{
\begin{tabular}{p{10mm}ll}\hline
Rank & Linguistic Pattern & $|Rels|$ \\\hline
\multicolumn{3}{l}{(A) Directly ($n_{patterns}=53$)} \\
1 & {[}{[}cause{]}{]}/N -nsubj cause/VB +dobj {[}{[}effect{]}{]}/N & 904,385 \\
2 & {[}{[}cause{]}{]}/N -nmod:with associated/VBN -acl {[}{[}effect{]}{]}/N & 892,908 \\
3 & {[}{[}cause{]}{]}/N -nsubj lead/VB +nmod:to {[}{[}effect{]}{]}/N & 783,860 \\
% 4 & {[}{[}cause{]}{]}/N -nsubj led/VBD +nmod:to {[}{[}effect{]}{]}/N & 724,978 \\
% 5 & {[}{[}cause{]}{]}/N -nsubjpass associated/VBN +nmod:with {[}{[}effect{]}{]}/N & 692,666 \\
\hline
\multicolumn{3}{l}{(B) Reverse-Engineered ($n_{patterns}=477$)} \\
1 & {[}{[}cause{]}{]}/N -nsubj led/VBD +nmod:to {[}{[}effect{]}{]}/N & 67,255 \\
2 & {[}{[}cause{]}{]}/N -nsubj produced/VBD +obj {[}{[}effect{]}{]}/N & 43,188 \\
3 & {[}{[}cause{]}{]}/N -nsubj brought/VBD +obj {[}{[}effect{]}{]}/N & 35,065 \\
% 4 & {[}{[}cause{]}{]}/N -nsubj caused/VBD +obj {[}{[}effect{]}{]}/N & 33,274 \\
% 5 & {[}{[}cause{]}{]}/N -nsubj resulted/VBD +nmod:in {[}{[}effect{]}{]}/N & 31,367\\
\hline
\end{tabular}
}
\caption{Top linguistic patterns from CauseNet's Wikipedia Dataset (A) Directly, and (B) Reverse-Engineered.
}\label{tab:top_patterns}
\end{table}
